Enabling Inference Privacy with Adaptive Noise Injection

User-facing software services are becoming increasingly reliant on remote servers to host Deep Neural Network (DNN) models, which perform inference tasks for the clients. Such services require the client to send input data to the service provider, who processes it using a DNN and returns the output predictions to the client. Due to the rich nature of the inputs such as images and speech, the input often contains more information than what is necessary to perform the primary inference task. Consequently, in addition to the primary inference task, a malicious service provider could infer secondary (sensitive) attributes from the input, compromising the client's privacy. The goal of our work is to improve inference privacy by injecting noise to the input to hide the irrelevant features that are not conducive to the primary classification task. To this end, we propose Adaptive Noise Injection (ANI), which uses a light-weight DNN on the client-side to inject noise to each input, before transmitting it to the service provider to perform inference. Our key insight is that by customizing the noise to each input, we can achieve state-of-the-art trade-off between utility and privacy (up to 48.5% degradation in sensitive-task accuracy with <1% degradation in primary accuracy), significantly outperforming existing noise injection schemes. Our method does not require prior knowledge of the sensitive attributes and incurs minimal computational overheads.

==> discussion.tex <==
\section{Discussion}

\subsection{Visualizing Preprocessed Inputs}
Fig~\ref{fig:transformed_inputs} visualizes the weights $w$ and the transformed inputs $x'$ produced by ANI for various inputs $x$ from the CelebA dataset for the smile detection task. Additionally, we visualize the transformed inputs $x'$ produced by Sieve as a point of comparison. Note that the spatial features of the input $x$ corresponding to high values of $w$ and $1-(\sigma/\sigma_{max})$ are preserved in the transformed representation $x'$. We make the following key observations:

\textbf{Hiding non-conducive features:} For the smile detection task, ANI produces a high value of the weights only near the mouth and low values everywhere else along the spatial dimensions of the image. Additionally, ANI chooses to retain information only along a single color channel (green) and hides the information in all the other color channels. By producing weight values that hide irrelevant parts of the input, ANI is able to produce a transformed representation $x'$, which is stripped of the information that is not pertinent to the primary classification task.

\textbf{Adaptivity to the input:} For the smile detection task, we ideally want to retain information closer to the mouth region. However, there can be significant variations in the spatial coordinates where the mouth of the person is found. The adaptive nature of ANI allows our method to customize the weights to capture this spatial variation and retain information corresponding to the mouth for each input image. In contrast, prior noise injection work which use a fixed noise distribution, has to resort to retaining a larger amount of spatial information to capture this variation, resulting in a worse utility-privacy trade off compared to ANI.  

\begin{figure}[htb]
	\centering
    %\epsfig{file=figs/examples.pdf, width=\textwidth}
    \epsfig{file=figs/examples.pdf, width=0.8\columnwidth}
	\caption{Comparing the noise masks produced by ANI with a recent prior work (\emph{Sieve}) for the smile detection task with CelebA dataset. ANI produces noise masks (weights $w$) that are tailored to the input, enabling ANI to obfuscate a greater fraction of the input. In contrast, Sieve produces a fixed noise mask, independent of the input. This adaptivity to the input enables ANI to achieve a better utility-privacy trade off compared to Sieve.}
	%Visualization of weight vectors $w$ and transformed inputs $x'$ produced by ANI corresponding to various inputs $x$ in the CelebA dataset for the smile detection task. ANI is able to obscure most of the irrelevant features of the input. Tailoring the noise by customizing the weight for each input allows ANI to achieve a better utility-privacy trade off compared to prior works.
    \label{fig:transformed_inputs}
\end{figure}


\subsection{Computational Overheads of ANI}~\label{sec:compute}
It is desirable to have low computational overheads for the network $f_w$ that is deployed on the client-side in ANI. This is because client devices like smartphones or smart home devices are likely to have low compute capabilities. To meet this requirement we designed the $f_w$ to have low computational overheads. For reference, $f_w$ only requires $5\%$ of the FLOPs required to evaluate $f_p$ for MNIST and FashionMNIST. This number is even lower at $<0.5\%$ for CIFAR-100 and CelebA datasets.
